Unicyclic graphs and the inertia of the distance squared matrix

A result of Bapat and Sivasubramanian gives the inertia of the distance squared matrix of a tree. We develop general tools on how pendant vertices and degree 2 vertices affect the inertia of the distance squared matrix and use these to give an alternative proof of this result. We further use these tools to extend this result to certain families of unicyclic graphs, and we explore how far these results can be extended.

==> abstract.tex <==
\begin{center}
    ABSTRACT
    
    \vspace{3em}
    
    FINDING PATTERNS IN THE INERTIA OF THE
        
    DISTANCE SQUARED MATRIX OF UNICYCLIC GRAPHS
    
    \vspace{3em}
    
    Kellon Sandall
    
    Mathematics Department
    
    Bachelor of Science
    
    \vspace{3em}
    
\end{center}

We analyze the spectrum of the distance squared matrix of a tree and give a relation between the inertia of the distance squared matrix and the structure of the tree. We take the result one step further and consider the addition of exactly one cycle in the tree. We obtain an expression for the inertia of the distance squared matrix of a cycle graph. We obtain a bound on the inertia of the distance squared matrix of an arbitrary unicyclic graph. 

==> acknowledgements.tex <==
\begin{center}
		ACKNOWLEDGEMENTS
		
		\vspace{3em}
\end{center}

This project wouldn't have come to fruition without the help of many people. I would like to thank my research advisor Dr. Mark Kempton for helping me understand matrix analysis better and helping me get past sticky points in my research. I would also like to thank Christian Howell for helping me with writing and proving various portions of the paper. I would also like to express gratitude to Dr. Ben Webb for talking with me about this paper in its various stages. I would like to thank Seth Larson who encouraged me to push through this project until the end. I am grateful for his friendship through the years and his view of my potential. Finally, I would like to thank my parents for their support and belief in me. 

==> sections/p_cycle_one_tree.tex <==
\section{A $p$-Cycle with exactly one tree connected to a vertex}

% THIS SECTION IS OLD AND NOT NEEDED ANYMORE.

% \iffalse
% The proof below is an old one. 

% \begin{proof}
% Let $T$ be a unicyclic graph on $n \geq 4$ vertices %This might need to change
% and assume the conclusion is true for all trees on fewer than $n$ vertices (but at least 3 vertices). If the diameter of the tree portion of the graph is 1 or 2, then
% \begin{equation*}
%     \Delta = \begin{bmatrix}
%         C & B \\
%         B^T & 4J - 4I
%     \end{bmatrix}
% \end{equation*}
% where $C$ is the distance squared matrix of the $p$-cycle, $B$ is the distance squared matrix for paths from the cycle to the tree and $4J - 4I$ is $(n - p) \times (n - p)$.

% $\Delta$ is equivalent (performing similar row and column operations) to 
% \begin{equation*}
%     \begin{bmatrix}
%         D & \textbf{0} \\
%         \textbf{0} & 4J - 4I
%     \end{bmatrix}
% \end{equation*}
% where $D$ is the result of creating the 0 matrices. We will have that $i_-(4J - 4I) = n - p - 1$ (-4 with a multiplicity of $n - p - 1$) and $i_+(4J - 4I) = 1$ ($4(n - p + 1)$).

% %Question: Do I need to go further with getting the eigenvalues of D?
% \end{proof}

% \fi
